Policy-as-Prompt: Rethinking Content Moderation in the Age of Large Language Models

Content moderation plays a critical role in shaping safe and inclusive online environments, balancing platform standards, user expectations, and regulatory frameworks. Traditionally, this process involves operationalising policies into guidelines, which are then used by downstream human moderators for enforcement, or to further annotate datasets for training machine learning moderation models. However, recent advancements in large language models (LLMs) are transforming this landscape. These models can now interpret policies directly as textual inputs, eliminating the need for extensive data curation. This approach offers unprecedented flexibility, as moderation can be dynamically adjusted through natural language interactions. This paradigm shift raises important questions about how policies are operationalised and the implications for content moderation practices. In this paper, we formalise the emerging policy-as-prompt framework and identify five key challenges across four domains: Technical Implementation (1. translating policy to prompts, 2. sensitivity to prompt structure and formatting), Sociotechnical (3. the risk of technological determinism in policy formation), Organisational (4. evolving roles between policy and machine learning teams), and Governance (5. model governance and accountability). Through analysing these challenges across technical, sociotechnical, organisational, and governance dimensions, we discuss potential mitigation approaches. This research provides actionable insights for practitioners and lays the groundwork for future exploration of scalable and adaptive content moderation systems in digital ecosystems.

==> tables/prompt_styles.tex <==
\setlength{\arrayrulewidth}{1pt} % Set the width of the outer border

\begin{table}[h!]
\centering
\begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{0.2\textwidth} 
                                   >{\raggedright\arraybackslash}p{0.18\textwidth} 
                                   >{\raggedright\arraybackslash}p{0.18\textwidth} 
                                   >{\raggedright\arraybackslash}p{0.18\textwidth} 
                                   >{\raggedright\arraybackslash}p{0.18\textwidth}}
\textnormal{\fontsize{6}{8}\selectfont Pr\ \ \ mpts that incite violence or hatred towards a, person or group, of people based on race religion gender identity or expression sex, ethnicity,, nationality sexual orientation veteran, status age disability or other characteristics associa\ \ \ ed with systemic discrimination or marginalization includes but may not be limited to: prai\ \ \ sing supporting, or calling for violence or exclusion, against a person or group of people based on the characteristics lis \ ted above, dehumanizing statements... 
} & 
\textnormal{\fontsize{6}{8}\selectfont - Prompts that incite violence or hatred towards individuals or groups are prohibited.  
- These prompts target characteristics such as:  
  - race 
  - religion  
  - gender identity or expression  
  - sex  
  - ethnicity  
  - nationality  
  - sexual orientation  
  - veteran status  
  - age  
  - disability  
  - other characteristics linked with systemic discrimination or marginalization  
- Prohibited actions include, but are not limited to:  
  - Praising, supporting, or calling for violence or exclusion against individuals or groups based on the aforementioned characteristics.  
  - Making dehumanizing statements...} & 
\textnormal{\fontsize{6}{8}\selectfont Policy that prohibits content inciting violence or hatred on grounds of race, religion, gender identity, sex, ethnicity, nationality, sexual orientation, veteran status, age, disability, or other marginalized traits includes, but is not limited to: endorsing or advocating violence or exclusion, dehumanizing statements...} & 
\textnormal{\fontsize{6}{8}\selectfont The policy is dedicated to addressing and regulating prompts that have the potential to incite or provoke acts of violence or expressions of hatred directed toward an individual or a group of individuals. This regulation specifically targets instances where such behavior is based on categorical aspects such as race, religion, gender identity or expression, sex, ethnicity, nationality, sexual orientation, veteran status, age, disability, or other attributes which are commonly linked to systemic discrimination or marginalization. The policy encompasses, but is not strictly limited to, behaviors such as: endorsing, supporting, or advocating for acts of violence or exclusion toward an individual or groups of individuals based on any of the aforementioned characteristics, making statements that dehumanize an...} & 
\textnormal{\fontsize{6}{8}\selectfont If a message encourages violence or hatred towards someone because of their race, religion, gender identity, sex, ethnicity, nationality, sexual orientation, veteran status, age, disability, or other similar traits, it's not allowed. This includes actions like praising, supporting, or demanding violence or exclusion of these individuals. It also involves saying dehumanizing things...} \\[5pt]
\multicolumn{1}{c}{\fontsize{8}{10}\selectfont Punctuated} & 
\multicolumn{1}{c}{\fontsize{8}{10}\selectfont Structured} & 
\multicolumn{1}{c}{\fontsize{8}{10}\selectfont Concise} & 
\multicolumn{1}{c}{\fontsize{8}{10}\selectfont Verbose} & 
\multicolumn{1}{c}{\fontsize{8}{10}\selectfont Annotator} \\
\end{tabularx}
\caption{\fontsize{8}{10}\selectfont Different styles for an excerpt of policy category: Hate.}
\label{tab:example}
\end{table}





